Language Bias in LVLMs: From In-Depth Analysis to Simple and Effective Mitigation

Large Vision-Language Models (LVLMs) extend large language models with visual understanding, but remain vulnerable to hallucination, where outputs are fluent yet inconsistent with images. Recent studies link this issue to language bias-the tendency of LVLMs to over-rely on text while neglecting visual inputs. Yet most analyses remain empirical without uncovering its underlying cause. In this paper, we provide a systematic study of language bias and identify its root in modality misalignment during training. Our analysis shows that both Visual Instruction Tuning (VIT) and Direct Preference Optimization (DPO) often prioritize textual improvements, which may cause LVLMs to overly lean toward language modeling rather than balanced multimodal understanding. To address this, we propose two simple yet effective methods: Language Bias Regularization (LBR) which mitigates language bias through regularization during instruction tuning, and Language Bias Penalty (LBP), which penalizes language bias in the DPO training process. Extensive experiments across diverse models and benchmarks demonstrate the effectiveness of our approach. LBR consistently improves performance on over ten general benchmarks, while LBP significantly reduces hallucination and improves trustworthiness. Together, these methods not only mitigate language bias but also advance the overall alignment of LVLMs, all without introducing any additional data or auxiliary models. Our code is publicly available at https://github.com/lab-klc/LVLM-Language-Bias.

==> table/human_evaluation.tex <==
\begin{table}[t]
\centering
\caption{Comparison of hallucination counts between DPO and Ours across different categories.}
\renewcommand{\arraystretch}{1.0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Method} & \textbf{Existence} & \textbf{Attribute} & \textbf{State} & \textbf{Number} & \textbf{Action} & \textbf{Relation} & \textbf{Sum of Hal.} \\
\midrule
DPO   & 33 & 17 & 15 & 48 & 9 & 15 & 137 \\
LBP  & 17 & 12 & 7  & 32 & 6 & 9  & 83  \\
VIT  & 95 & 6 & 2 & 32 & 12 & 8 & 155 \\
LBR & 73 & 5 & 2  & 27 & 9 & 5  & 121  \\
\bottomrule
\end{tabular}
}
\label{tab:human_LBR}
\end{table}


==> table/hyper-para-ablation.tex <==
\renewcommand{\arraystretch}{1.2} % 调整行间距
\begin{table}[t]
\caption{Performance of different $\alpha$ values on various VQA benchmarks. Best results are in \textbf{bold}, second-best are \underline{underlined}.}
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{$\alpha$} & MME & SQA & \textbf{VQA$^\text{Text}$} & CocoCap \\
\midrule
0 & 1490 & 66.8 & 45.8 & 110.6 \\
1e-3 & 1492 & 69.9 & 45.7 & 110.8 \\
1e-4 & 1517 & 68.3 & 45.6 & 116.3 \\
1e-5 & \textbf{1525} & 69.4 & \textbf{46.0} & 112.1 \\
1e-6 & 1484 & \textbf{70.7} & 45.6 & 110.1 \\
1e-7 & 1457 & 68.9 & 46.0 & 112.2 \\
\bottomrule
\end{tabular}

\label{tab:alpha}
\end{table}


==> table/larger_lbp.tex <==
\renewcommand{\arraystretch}{1.0}
\setlength{\aboverulesep}{0.5pt}
\setlength{\belowrulesep}{0.5pt}
\begin{table}[t]
    \centering
    \caption{Scalability analysis on a larger preference dataset (30k samples from VLFeedback). LBP demonstrates consistent improvements over DPO baselines across multiple hallucination benchmarks.}
    \label{tab:scalability_vlfeedback}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|cc|cccc|cc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} 
      & \multicolumn{2}{c|}{\textbf{MMHalBench}} 
      & \multicolumn{4}{c|}{\textbf{AMBER (Generative)}} 
      & \multicolumn{2}{c|}{\textbf{AMBER (Discriminative)}} 
      & \multicolumn{2}{c}{\textbf{Object HalBench}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
      & Score $\uparrow$ & HalRate $\downarrow$ & CHAIR $\downarrow$ & Cover $\uparrow$ & Hal $\downarrow$ & Cog $\downarrow$ 
      & Acc. $\uparrow$ & F1 $\uparrow$ & CHAIR$_s$ $\downarrow$ & CHAIR$_i$ $\downarrow$ \\
    \midrule
    DPO & 2.80 & 0.54 & 5.8 & \textbf{53.5} & 31.9 & \textbf{2.7} & 79.5 & \textbf{85.9} & 33.5 & 18.5 \\
    DPO$_\text{M}$ & 3.02 & 0.41 & 5.7 & 50.5 & 27.9 & 2.8 & 79.8 & 85.8 & 31.2 & 17.5 \\
    \rowcolor{gray!20}
    \textbf{LBP (Ours)} & \textbf{3.05} & \textbf{0.39} & \textbf{5.4} & 51.1 & \textbf{26.6} & \textbf{2.7} & \textbf{79.9} & \textbf{85.9} & \textbf{30.1} & \textbf{17.1} \\
    \bottomrule
    \end{tabular}}
\end{table}
